Dependency Dialogue Acts -- Annotation Scheme and Case Study

In this paper, we introduce Dependency Dialogue Acts (DDA), a novel framework for capturing the structure of speaker-intentions in multi-party dialogues. DDA combines and adapts features from existing dialogue annotation frameworks, and emphasizes the multi-relational response structure of dialogues in addition to the dialogue acts and rhetorical relations. It represents the functional, discourse, and response structure in multi-party multi-threaded conversations. A few key features distinguish DDA from existing dialogue annotation frameworks such as SWBD-DAMSL and the ISO 24617-2 standard. First, DDA prioritizes the relational structure of the dialogue units and the dialog context, annotating both dialog acts and rhetorical relations as response relations to particular utterances. Second, DDA embraces overloading in dialogues, encouraging annotators to specify multiple response relations and dialog acts for each dialog unit. Lastly, DDA places an emphasis on adequately capturing how a speaker is using the full dialog context to plan and organize their speech. With these features, DDA is highly expressive and recall-oriented with regard to conversation dynamics between multiple speakers. In what follows, we present the DDA annotation framework and case studies annotating DDA structures in multi-party, multi-threaded conversations.

==> jai_related_work_saved.tex <==
\section{Related Work}
\jmf{Shorten}
Our work is mainly related to two lines of research: dialogue acts, rhetorical relations. However, our focus is on multi-party multi-threaded dialogue, especially the multi-relational response structure beyond dialogue acts and rhetorical relations.
\subsection{Dialogue Acts}
%Dialogue acts describe the communicative actions for utterances in a dialogue, such as questions, promises, requests, and greetings.
The idea that each utterance is performing an action by the speaker was due originally to the philosopher Wittgenstein~\cite{wittgenstein2010philosophical}. 
Speech act theory by Austin~\cite{austin1975things} and his student John Searle~\cite{searle1969speech} was one of the first attempts at developing a set of communicative actions. Then many researchers~\cite{allwoodactivity,cohen1990intentions,hancher1979classification} noticed that a major problem with speech act theory is that it attempts to capture an utterance's purpose(s) with one label. However, multi-functionality is common in dialogues, especially in multi-party multi-threaded dialogues. One of the most sophisticated research on multi-dimensional and multifunctionality related to DDA is Dynamic Interpretation Theory~(DIT)~\cite{bunt1999dynamic} and DIT++ schema~\cite{bunt2006dimensions, bunt2009dit++}) who combines the concepts from above various alternative schemas, and provides precise and consistent definitions for its communicative functions and dimensions. Based on the comprehensive DIT++ taxonomy on dialogue acts, ISO 24617-2~\cite{bunt-etal-2010-towards, bunt-etal-2012-iso, bunt-etal-2020-iso} proposed a semantically-based standard for dialogue annotation, including both dialogue acts and the relations between them. Another line of research originated from DAMSL~(Dialogue
Act Markup in Several Layers)~\cite{allen1997draft, core1997coding} addresses this problem by allowing an utterance simultaneously perform multiple actions in multiple independent layers (\emph{Communicative-Status}, \emph{Information-Level}, \emph{Forward Looking Function}, \emph{Backward Looking Function}), and each layer involves multiple sub-divided tags~(around 3, 4, 12, 13 leaf tags for each layer). With its focus on multi-dimensionality and domain independence, DAMSL inspired various extensions of dialogue act annotation, such as SWBD-DAMSL~\cite{jurafsky1997switchboard} and COCONUT~\cite{di1998coconut}. One issue of DAMSL is that thousands of combinations of DAMSL tags make the search space for both human and automatic annotation a huge challenge. To address this, SWBD-DAMSL, which is a version of DAMSL specially adapted for the annotation of the Switchboard Corpus~\cite{godfrey1992switchboard} were introduced, where only 220 combinations~(including 28 new tags not in DAMSL) are used and clustered into 42 mutual exclusive tags(flatten multi-functional labels). The reduced search space(42 mutually exclusive tags) was well adapted to the initial goals of automatic annotation of dialogue acts and the use of dialogue act specific language models in speech recognition~\cite{stolcke2000dialogue}. However, it partially sacrifices the freedom and expressiveness on multi-functionality. This echos with the cross-dimension phenomenon discussed in DAMSL standard~\cite{allen1997draft} and SWBD-DAMSL\cite{jurafsky1997switchboard} which is considered a trade-off of annotaiton scalability versus expressiveness. 
% \jzc{TODO: rephrase for the multi-dimensional; switch order of DIT and DAMSL; why swbd-DAMSL; why not tagging}  
In our work, we follow SWBD-DAMSL's approach by using an augmented version of SWBD-DAMSL's flattened DA tag set as the elements of DDA's dialogue structure space. Nevertheless, we made two augmentations: first, DDA handles multi-functionality phenomenon with multi-label and multi-dependency; second, DDA resolves the response structure, which not only unveils a deeper discourse structure in conversations but also anchors the dialogue act and discourse relations into context, which is fundamenally different than tagging schemes; In limited practice, we find the efficiency of annotating DDA to be comparable to SWBD-DAMSL.
% \jic{@Jon, given the related work , please clarify here, what is our consideration on multi-functionality, or balancing the annotating speed?
% we just follow xxx to handle the multi-functionality issue, and extend xx for specific purposes.}

%Dialogue acts can be interpreted formally as update operations, to be applied to the information states of the interacting participants; this view is commonly known as the ‘information-state update’ or ‘context-change’ approach to the analysis of dialogue – see e.g. Traum & Larsson (2003); Bunt (2000; 2011).
% \jic{@Jon, please check the ISO document here(sec 2.4, 4.1, \url{https://hal.inria.fr/inria-00544997/document} also the DASML papers, it seems DASML is designed for handling multi-labels issues. and ISO is also aware of the multi-functionality for dialogue acts and it seems also considering this?  }

%Besides the dialogue acts, relations between dialogue acts has also been considered when designing the dialogue acts, such as forward-looking and backward-looking functions.

\subsection{Rhetorical relations in Multi-party Dialogue}
Previous works on structured analysis for multi-party dialogue~\cite{kummerfeld_large-scale_2019, elsner_you_2008} mainly focused on simple thread disentanglement, rather than analyzing the resulting rhetorical structures).\jic{@brendon, could you add more here to demonstrate the current status of response structures in multi-party dialogue} In this work, we mainly focus on the rhetorical structures in multi-party dialogue.  Given rhetorical relations~(discourse relations) has been widely studied in various discourse theories, researchers widely introduce the existing discourse annotation framework for dialogue structured analysis. Rhetorical structure theory(RST)~\cite{mann1988rhetorical}, Discourse Representation Theory~(DRT)\cite{kamp2011discourse}, Hobbs' theory of discourse \cite{hobbs1990literature}, and Penn Discourse Treebank~(PDTB)~\cite{prasad2008penn} framework are the four most influential framework has been used in dialogue analysis. An RST tree is built recursively by connecting the adjacent discourse units, forming a hierarchical structure covering the whole text.   RST Bank~\cite{carlson2003building} created a reference corpus for community-wide use, while~\cite{stent-2000-rhetorical} provides a practical analysis on annotating dialogue with RST. Similar to the RST framework, the Segmented Discourse Representation Theory~(SDRT) SDRT~\cite{asher2003logics}(based on DRT) also provides a hierarchical structure of text organization with full annotation. For example, DISCOR corpus~\cite{reese2007reference}, the ANNODIS corpus~\cite{afantenos2012empirical}, and the STAC~\cite{asher-etal-2016-discourse} use directed acyclic graphs that allow for multiple parents, but not for crossing. 
Based on Hobbs’ theory, Discourse Graphbank~\cite{wolf2005representing} allows for general graphs that allow multiple parents and crossing. Unlike the above frameworks, PDTB adopts a theory-neutral approach to the annotation, which does not aim at achieving complete annotation of the text but focuses on local
discourse relations anchored by structural connectives or discourse adverbials. This theory neutrality makes no commitments to what kinds of high-level structures may be created from the low-level annotations of relations and their arguments, thus it permits more freedom of investigating complex dependency structures in multi-party multi-threaded dialogue. Furthermore, ISO DR-Core also follows the theory-neutral stance in PDTB, annotating only low-level discourse relations that can then be annotated further to project a higher-level tree or graph structure, depending on one’s theoretical preferences. Last but not least, DDA follows PDTB's discourse relation taxonomy since it has been demonstrated effective in annotation practice to yield good annotator agreement.
% \jic{@Jon, we just adopt PDTB because of ISO and some other benefits, please help here. Then if possible, write the limitation of just using PDTB for mulit-party dialogue, what is our contribution here}

%The theory by Grosz and Sidner (1986) believes that that discourse structure is composed of three separated but interrelated components: linguistic structure, intentional structure and attentional structure. These three aspects capture discourse phenomena in a systematic way, and other discourse theories may be related to this theory in some way. For instance, the Centering Theory (Grosz et al., 1995) and the entity-grid model (Barzilay and Lapata, 2008) focus on the attentional structure, and the Rhetorical Structure Theory (RST) (Mann and Thompson, 1988) focuses on the intentional structure.

% \bdk{Would it make sense to arrange this section as discussing three (or however many) perspectives there are on annotating multi-party dialogue? e.g: \begin{enumerate}
%     \item Semantic annotation of dialogue (e.g. ISO): speech is composed of communicative functions, which can be broken down into "elementary update functions" \cite{bunt_semantics_2011}, which have an intended functional effect on the information state of an addressee. (this claim needs more research:) Relations between functional segments/utterances are only added when needed for interpreting that communicative function. Note: this does not apply to the rhetorical relations in ISO, which would fit in the next sub-section, but these are not the primary purpose of ISO and seem more like an effort to incorporate other existing work (e.g. ISO 24617-2 does not define its own rhetorical elation set).
%     \item Rhetorical structured annotation of dialogue (e.g. RST, RST4Dialog, SDRT, etc.): Connecting discourse units by their rhetorical relationships
%     \item Response structure: annotation efforts simply label which utterance(s) an utterance-of-interest responds to. Connected components are extracted to form threads for down-stream conversational tasks. (Not sure if this is worth highlighting as an annotation scheme or how to discuss, since its value in previous work seems much more focused on simply separating threads, rather than analyzing the resulting structure) \cite{kummerfeld_large-scale_2019, elsner_you_2008} + a few more datasets and many methods papers. 
% \end{enumerate}
% Unsure: Where does SWBD-DAMSL fit? Are these categories distinct enough and representative of everything we want to cover in the section?}
%\jzc{SWBD-DAMSL cares the ``shallow discourse structure'' instead of ``deep'' in the sense that the response structure and communicative function structure are assumed to be between adjacent pairs, which is a degenerated case of ISO and DDA. They made the choice for scalability. SWBD-DAMSL thus focus on the dialog act tag set design instead of the structure and the coverage rate of the dialog act space should be considered relatively full(ISO and other DA frameworks are not shifting too much from SWBD-DAMSL's tag set). I'm rephrasing from the intro part of SWBD-DAMSL manual.}
% In this section, we discuss three existing corpora and their schemes: Switchboard corpus(SWBD-DAMSL), The ICSI Meeting Recorder Dialog Act (MRDA) Corpus and DialogBank corpus. \\
% Chronologically among the three, SWBD-DAMSL is the first that systematically defined their annotation scheme. It is considered one of the most valuable resource to study the dialogue phenomenons between two dialogue participants on telephone. The main goal of SWBD-DAMSL is to create a comprehensive framework for modeling DAs in a data driven way, meaning the DAs are not only described and defined through the annotation guidelines but also manifested from annotations. The core feature SWBD-DAMSL adopted is the DAMSL DA Tag set[cite Core and Allen 1997], which lead to fact that the majority of the DA classes overlaps with Core and Allen's work. Meanwhile, SWBD-DAMSL's labeling differs from DAMSL for "content- and task-related" aspect and it further simplified the tag set. They also adopted multidimensional annotations to cover other orthogonal aspects of the functionality of the dialogue such as "Task-management" and "Communication-management". Overall, SWBD-DAMSL scheme consolidated the 220 possible combinations of DAMSL labels into 42 classes for practical reasons, which include but not limited to increasing the inter-annotator-aggrement and scale of coverage. Similar to DAMSL, SWBD-DAMSL scheme also organized the 42 tags into orthogonal dimensions except that "Communicative-status" is not considered one of the dimension comparing with DAMSL. 
% We show statistics of SWBD-DAMSL corpus in Table 1. \\
% \\
% Later, International Computer Science Institute(ICSI) developed a new Dialog Act annotation scheme for multi-party meeting records(MRDA). This annotation scheme incorporated most DA tags from SWBD-DAMSL but also introduced modifications to reflect multi-party nature of their domain. We list the major changes made in MRDA comparing with SWBD-DAMSL. First, MRDA redefined tag set and recategorized them into 13 groups instead of 5[cite MRDA manual]. There are sub categories in the "Response" group and "Restated Information" group, which makes their tag set a two tiers hierarchical structure. In terms of labeling, MRDA introduced a 3 dimensional tagging scheme, the general tag, specific tag, and disruption forms, in which general tag is mandatory, while specific tag and disruption forms are optional. The 3 dimensions are another way of clustering the MRDA DAT tag set. Further, the specific tags can contain multiple tags, which the other two dimension are labeled exclusively within their tag set. We summarize MRDA's tag set overlapps and differences compared with SWBD-DAMSL in Table 2.\\
% \\
% Another dialogue resources we closely follow is the DialogBank developed by Bunt et al.. The annotation scheme forms ISO 24617-2 standard(ISO-standard hereafter) for more than DA annotations. The ISO-standard intend to form a comprehensive annotation standard to cover multiple dialogue phenomena, such as Dialog Acts, Rhetorical Structures, dependency relations and modalities. Compared with SWBD and MRDA whose main focus lies within Dialog Acts. In terms of the DA labeling, ISO-standard use multiple dimensions to encode DAs instead of directly incorporating tag sets from SWBD and MRDA. Specifically, ISO-standard uses ``semantic content'' field combined with ``Communicative function'' field and ``qualifier'' field to encode Dialog Act that conceptually corresponding to DAs. The map from SWBD-DAMSL to ISO-standard has been studies by [citation], in which they show the transformation from SWBD-DAMSL tag to ISO-standard does not have a one to one map. The overall SWBD-DAMSL to DA tag ISO DA type one-to-one and many-to-one translatable rate is 83.97\% in terms of utterance count.


\subsection{Annotating Response Structure Graphs}
\bdk{Outline: (1) present task, (2) discuss available corpora, (3) TODO: compare our notion of response/reply with theirs, and discuss how all our edges are labeled.}
Another line of work aims to improve conversational understanding systems by uncovering the response dependencies between utterances in multi-party speech \cite{aoki_wheres_2006} or online chat \cite{elsner_you_2008, kummerfeld_large-scale_2019, du_discovering_2016}. Given dialogue segmented into utterances, the task is to connect an utterance of interest (UOI) with all previous utterances to which it responds. The resulting connected components form dialogue threads which can be understood individually in downstream systems. \cite{kummerfeld_large-scale_2019} present one of the largest available corpora annotated with reply structure graphs, consisting of 77,653 messages from the Ubuntu Internet Relay Chat (IRC). Our notion of response dependency is similar to this line of work with a few key differences. (1) All of our dependencies are labeled with the dialogue act and/or rhetorical relation initiated in the responding utterance. (2) In many cases, the direction of the relation edge denotes the semantic roles of each utterance (e.g. as in Answer $\to$ Question). (3) An utterance of interest can respond to any number of previous utterances using any number of labels. 
% point below probably needs revision/clarification
(4) Though relatively rare in dialogue, we do not forbid forward-looking dependencies, as one might encounter in monologues, where a participant is organizing their speech toward a planned utterance. But for consistency purpose, we prefer the dependency relations to reflect real time interpretation of the "triggering" and "response" structure and encode the directionality with aforementioned dual tags.
% \jzc{(5) An UOI is considered to have response structure(s) if it is continuing a thread of conversation even if the addressee(s) of the UOI is not the speaker of the tiggering utterance(s)}


==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. OConnell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...´': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}

